Groebner techniques for low degree Hilbert stability

We give a method for verifying, by a symbolic calculation, the stability or semistability with respect to a linearization of fixed, possibly small, degree $m$, of the Hilbert point of a scheme $X \in {\mathbb P}(V)$ having a suitably large automorphism group. We also implement our method and apply it to analyze the stability of bicanonical models of certain curves. Our examples are very special, but they arise naturally in the log minimal model program for $\bar{\mathcal M}_g$. In some examples, this connection provides a check of our computations; in others, the computations confirm predictions about conjectural stages of the program.

==> codesamples.tex <==
\input{newgrobnerpreamble}

\externaldocument{newgrobner}

\begin{document}

\def\normallinespread{1.15}
\linespread{\normallinespread}\normalfont\selectfont
\lineskiplimit=-0.08cm

\pagenumbering{arabic}

\title{Code samples to accompany ``Gr\"{o}bner techniques for low degree Hilbert stability''}

\author{Ian Morrison}
\address{Department of Mathematics\\ Fordham University\\ Bronx, NY 10458}
\email{morrison@fordham.edu}

\author{David Swinarski}
\address{Department of Mathematics\\ University of Georgia\\ Athens, GA 30602}
\email{davids@math.uga.edu}

\subjclass[2000]{Primary 14L24, 14H10 \\Secondary 14D22, 13P10}
\keywords{Hilbert stability, state polytope}

\date{\today}

\maketitle

This file consists mainly of annotated code samples for performing various calculations discussed in our paper ``Gr\"{o}bner techniques for low degree Hilbert stability'' (available at \textbf{\Large point to arxiv once we post}) and linked to from that paper. These examples are intended to give readers not familiar with some of the packages we use models for calculations needed in our examples. We claim no originality---nor even any cleverness in coding. We have also included a few lengthy ideal descriptions omitted from the paper.

\codesample{ideals}{Ideals used in our paper}  Here we record some ideals used in our calculations, but, to save space, not listed in the paper.

\codesampleideal{ellipticbridgeideal}{The ideal $\mathcal{I}'$ of the elliptic bridge in Example~\ref{ellbr}}
Recall that this ideal is given in coordinates diagonalizing the two generating automorphisms.
\begin{eqnarray*}
\mathcal{I}' & = & 
(DG+GI,CG-GJ,CG+GJ,BG-GK,BG+GK,AG-GL,AG+GL,DF+FI,CF-FJ, \\
&&CF+FJ,BF-FK,BF+FK,AF-FL,AF+FL,E^2-EF-2EH-FH+H^2, \\
&&E^2-DF-H^2+FI, DE-DH+EI-HI,CE-CH-EJ+HJ,CE-CH+EJ-HJ,\\
&&BE-BH-EK+HK,  BE-BH+EK-HK, AE-AH-EL+HL,AE-AH+EL-HL,\\
&&-DE+E^2+DH+2EH+H^2+EI-HI, DE-F^2-G^2+DH-EI-HI,\\
&&DE+DH+EI+HI,CE+CH-EJ-HJ,CE+CH+EJ+HJ, BE+BH-EK-HK,\\
&&BE+BH+EK+HK,AE+AH-EL-HL,AE+AH0+EL+HL,BD-BI-DK+IK, \\
&&BD-BI+DK-IK,AD-AI-DL+IL,AD-AI+DL-IL,\\
&&-CD+D^2+CI+2DI+I^2-DJ+IJ, BD+BI-DK-IK,BD+BI+DK+IK,\\
&&AD+AI-DL-IL,AD+AI+DL+IL,  C^2-CD+D^2-CI-I^2-2CJ-DJ-IJ+J^2,\\
&&BC-BJ-CK+JK,BC-BJ+CK-JK,AC-AJ-CL+JL, AC-AJ+CL-JL,\\
&&B^2-BC-BJ-2BK-CK-JK+K^2,B^2-AC-AJ-K^2+CL+JL, \\
&&-AB+B^2+AK+2BK+K^2+BL-KL,2A^2-BC-BJ+CK+JK+2L^2)
\end{eqnarray*}

\codesampleideal{g2wpideal}{The ideal $I$ of the genus 5 nodal curve in with a genus $2$ Weierstrass tail in Example~\ref{g2wp}}
\begin{eqnarray*}  I &  = &  (gl,fl,el,dl,cl,bl,al,gk,fk,ek,dk,ck,bk,ak,\\
&&gj,fj,ej,dj,cj,bj,aj,gi,fi,ei,di,ci,bi,ai,\\
&&g^2-fh,fg-eh,eg-dh,dg-ch,ag-bh,f^2-dh,ef-ch,df-cg,\\
&&af-bg,e^2-cg,de-cf,ae-bf,d^2-ce,ad-be,ac-bd,\\
&&b^2+c^2-eh,ab+cd-fh,a^2+ce-gh,\\
&&j^2-ik,ij-hk,i^2-hj,hi-k^2-l^2) \label{genus2tailideal}
\end{eqnarray*}

\codesampleideal{g2nonwpideal}{The ideal $I$ of the genus 5 nodal curve with a general genus $2$ tail in Example~\ref{g2nonwp}}
\begin{eqnarray*} I(C) &  = & (gl,fl,el,dl,cl,bl,al, gk,fk,ek,dk,ck,bk,ak, \\
&& gj,fj,ej,dj,cj,bj,aj,gi,fi,ei,di,ci,bi,ai, \\
&& g^2-fh,fg-eh,eg-dh,dg-ch,ag-bh,f^2-dh,ef-ch,df-cg, \\
&& af-bg,e^2-cg,de-cf,ae-bf,d^2-ce,ad-be,ac-bd, \\
&& b^2+c^2-eh,ab+cd-fh,a^2+ce-gh\\
&& k^2-jl,hk-il,hj-ik,i^2-jk-2hl)\\
\end{eqnarray*}


\vfill \eject

\codesample{pluckercode}{Computing Pl\"{u}cker coordinates in \mtwonocite}

{To compute the Pl\"ucker coordinates of Example~\ref*{pluckerexample} we proceed as follows.
\linespread{1}\normalfont\selectfont%	
\begin{verbatim}
i1 : R = QQ[a..c];
i2 : I = intersect(ideal(c-3*a,b-2*a),ideal(a-5*b,c+4*b));
i3 : G = flatten entries super basis(2,I);
i4 : B = flatten entries basis (2,R);
i5 : M = matrix apply(#G, i-> apply(#B, j -> coefficient(B_j,G_i)))
o5 = | 11 -19 9  0   0   0  |
     | 0  1   0  -19 9   0  |
     | 0  0   11 0   -19 9  |
     | 0  0   0  12  -5  -2 |
i6 : flatten entries gens minors(4,M)
o6 = {15972, -6655, 27588, 1573, -25289, -2662, -13068, -4598, 
     18634, 10043, 2178, -11979, -6655, 11495, -5445}
i7 : gcd(oo)
o7 = 121
i8 : o6/o7
o8 = {132, -55, 228, 13, -209, -22, -108, -38, 154, 83, 18, -99, -55, 95, -45}
\end{verbatim}}

\noindent The order in which \mtwonocite\ lists the basis of $\bigwedge^{4} S_{2}$ does not match the convention used in our paper.  Note also that, in \mtwonocite, we computed the intersection of the two ideals, rather than the product.  The result is not the ideal we computed by hand, but its saturation.  The two Hilbert matrices are different but row-equivalent, and the two sets of Pl\"{u}cker coordinates agree up to a multiple of 121 in each coordinate (that we supressed in our listing), hence represent the same point in $\Pro^{14}$.  

\vfill\eject
\codesample{usingstatepolytopepackage}{Using the package \texttt{StatePolytope} in \mtwonocite}

Here we show how to use the package \texttt{StatePolytope} in \mtwonocite.

\begin{verbatim}
i1 : loadPackage("StatePolytope");
i2 : R=QQ[a..d];
i3 : I = ideal(a*c-b^2, a*d-b*c, b*d-c^2);
i4 : initialIdeals(I)
o4 = {{b*d, a*d, a*c}, {c^2, a*d, a*c}, {c^2, b*c, a*c, a^2*d}, {c^2,
b*c, b^3, a*c}, {c^2, b*c, b^2}, {b*d, b^2, a*d}, {b*d, b*c, b^2,
a*d^2}, {c^3, b*d, b*c, b^2}}
i5 : statePolytope(2,I)
i6 : statePolytope(3,I)
\end{verbatim}
To see $\State_m(I)$ for larger values of $m$, see Kapranov-Sturmfels-Zelevinsky, page 202.  Note that they compute state polytopes using monomials outside the initial ideal rather than inside, but it is simple to convert between the two conventions: simply subtract each vertex from the vector $\frac{((m+N-1)!m}{m!N!} (1,\ldots,1)$.
\vfill\eject
\codesample{Nspanningideals}{Testing whether N ideals span the barycenter}
If a point $Q$ is contained in a polytope $\mathcal{P} \subset \R^n$, then there exists a set of $n$ vertices $\{v_{j}\}_{j=1}^{n}$ of $\mathcal{P}$ such that $Q$ is contained in $\ConvHull \{ v_j \}$.  

In our Monte Carlo calculations, of course, it is more difficult to find exactly $n$ points whose convex hull contains the barycenter, but the calculations required are easier: rather than calling polymake or another convex geometry package, we can test this containment using linear algebra.

Let $L$ be the list of $n$ initial ideals.  Below we check whether $\{\State_3(I_j) \}$ contains $\bary_{3}$ in its convex hull.
\begin{verbatim}
i1 : R=QQ[a..i];
i2 : L = {
{a*h^2, d*f^3, a*f^2, d*g, c*d, a*g, g*h^2, c*h^2, b*h, a*e, h*i, b*f, e*h, f*i,
 c*f, e*f, b^2, b*i, b*g, i^2, b*c, b*e, c*i, c*g, e*i, e*g, c^2, c*e, e^2}, 
{b^3, e*h, b*h, b^2*c, a*b^2, c*e, a*e, e*g, b*g, f^2, f*h, d*f, c*f, a*f, f*g,
 d*h, d^2, c*h, g*h, c*d, a*d, d*g, c^2, a*c, a^2, c*g, a*g},
{d^4, d^2*g, a*e^2*i, c*d^2, d*g*h, a*g, c*e, c*d*h, e*f, b*e, d*f, d*i, b*d, a*f,
 h^2, c*g, b*g, f*h, h*i, c^2, b*h, c*f, c*i, b*c, f^2, f*i, i^2, b*f, b*i, b^2},
{b^5*i^2, c^5*f, c^3*e^2, b^2*e, c^2*e*f, b*e^2, a*c, b*f, a*i^2, a*e, e^3, c*f^2,
 a*f, e^2*f, b*h, b*d, c*h, b*g, c*d, f^3, c*g, a*d, e^2*h, a*g, d*e, h*i, e*g,
 d*i, f*h, d*f, f*g, h^2, d*h, d^2, g*h, d*g}, 
{c^4, a*b*f, b^2*f*h, a^2*f, a*c, a*f*h, c*h, a*i, c*e, c*d, b*e, b*d, a*e, a*d,
 c*g, b*g, i^2, a*g, h*i, e*i, h^2, e*h, d*h, e^2, d*e, d^2, g*h, e*g, d*g},
{b*f, b*e, a*d, c^2, c*f, c*e, e^2, d*h^2, d*g, e*h, a*c, b*g, a*f, a*e, b*i,
 c*h^2, f*h^2, c*g, e*g, c*i, e*i, a^2, g*h, h*i, a*g, a*i, i^2}, 
{d^3, c*d^2, c^2, b*g*h, b*e, d*e, c*e, b*f, d*f, c*f, i^2, e^2, a*g, f*i, e*f,
 a*d, a*c, d*h, c*h, f^2, a*i, a*e, h*i, e*h, a*f, f*h, h^2}, 
{b*d, c*e, c*f, b^2, a*d, c*g, b*e, b*f, e^2, d*h, b*i, e*f, a*e, d*g^2, b*g, a*f,
 e*g, a*i, i^2, a*g, e*h, f*h, h*i, g*h, h^2},
{b^3*e^3, b^4, c*f*h^2, b^3*c, c^3, e^2*f, d*h^2, c^2*f, a*b^2, e*f^2, c*f^2, b*f,
 a*e, a*c, f^3, d*e, b*d, h*i, c*d, a*f, e*i, e*g, b*i, a^2, c*i, b*g, c*g, d*f,
 a*d, f*i, a*i, a*g, d^2, d*i, d*g, i^2}
};
i3 : m=3;
i4 : Z = apply(#L, i -> subhp(m,ideal(L_j)));
i5 : bary = apply(9,i -> sum(Z_0)/9);
i6 : Z = transpose matrix Z;
i7 : v = (Z^-1) * matrix(transpose {bary}); 
i8 : apply(9, i -> v_0_i >=0) == apply(9, i -> true)
\end{verbatim}

In line \texttt{i4}, we create a matrix whose rows are the $\thst{3}{rd}$ Hilbert points of the initial ideals contained in the list \texttt{L}.  In line \texttt{i5}, we create the barycenter $\bary_{3}$.  Lines \texttt{i6} and \texttt{i7} write $\bary_{3}$ in the basis given by the $\thst{3}{rd}$ Hilbert points, and call this answer \texttt{v}. Finally, in line \texttt{i9}, we check that all coordinates of \texttt{v} are nonnegative.  


\vfill\eject
\codesample{curveequations}{Writing equations for curves in \Magmanocite}
Here we demonstrate how to get equations of a hyperelliptic curves under an embedding of the form $|aK+bP|$.  Specifically, we take $C = \wiman{3}$ and the linear series $|2K+2P|$ where $P$ is the point at infinity.

\begin{verbatim}
L<z>:=CyclotomicField(14);
R<x>:=PolynomialRing(L);
C:=HyperellipticCurve(x^7-1);
K:=CanonicalDivisor(C);
P:=C![1,0,0];
D:=2*K+2*Divisor(P);
phi:=DivisorMap(D);
WP2<x,y,z>:=Domain(phi);
P7<a,b,c,d,e,f,g,h>:=Codomain(phi);
phi;
Ideal(phi(C));
\end{verbatim}

Note that in writing the resulting equations in Example~\ref{g2wp}, we have reordered the variables to conveniently attach the genus $2$ tail.

\vfill\eject
\codesample{scrollequations}{Equations of scrolls in \mtwonocite}
In our paper, we see that ideals of bicanonical curves can be written as the ideal of a scroll plus some additional quadrics.  

We briefly mention that there is an easy way to get the ideal of such scrolls.

Take for instance the genus 4 Wiman curve $\wiman{4}$.  The ideal $I_{S}$ for the associated scroll can be obtained with the \mtwonocite\ commands
\begin{verbatim}
M = matrix {{i,g,f,e,d,c,b},{h,f,e,d,c,b,a}};
IS = minors(2,M)
\end{verbatim}

\vfill\eject
\codesample{mapleprox}{Computing the proximum with \texttt{Convex} in \texttt{Maple}}

Here is an example of how to find the proximum (closest point on a polytope to a point outside it) using the package \texttt{Convex} in \texttt{Maple}.  
\begin{verbatim}
with(convex):
P:=convhull([0,0],[1,0],[0,1],[1,1]):
Q:=Vector([2,0]):
proximum(P,Q);
quit:
\end{verbatim}

\vfill\eject
\codesample{wimanweiertailmultfree}{Checking multiplicity freeness in \Magmanocite}

Here is a sample code sample showing how to check that a reducible Wiman is multiplicity free in \Magmanocite. 

\begin{verbatim}
K<z>:=CyclotomicField(140);
u:=z^14;
t:=z^10;
GL12K:=GeneralLinearGroup(12,K);
D1:=DiagonalMatrix([t^5,t^3,t^10,t^12,t^0,t^2,t^4,t^6,t^6,t^6,t^6,t^6]);
D2:=DiagonalMatrix([u^8,u^8,u^8,u^8,u^8,u^8,u^8,u^8,u^6,u^4,u^2,u^7]);
G:=sub<GL12K | D1,D2>;
Gmod:=GModule(G);
chi:=Character(Gmod);
X:=CharacterTable(G);
Decomposition(X,chi);
\end{verbatim}

\section*{Software Packages Referenced}
\begin{biblist}[\setcounter{bib}{0}]
	\bib{Convex}{article}{
		author={Franz, Matthias},
		title={Convex: a Maple™ package for convex geometry},
		date={2006},
		note={Version 1.1.2},
		eprint={\href{http://www-fourier.ujf-grenoble.fr/~franz/convex/}{\texttt{http://www.fourier.ujf}-\texttt{grenoble.fr/\~{}franz/convex/}}},
	}
	\bib{Gap}{article}{
		author={The GAP~Group},
		title={\texttt{\upshape GAP}: Groups, Algorithms, and Programming, a system for computational discrete algebra},
		date={2008},
		note={Version 4.4.11},
		eprint={\neturl{http://www.gap-system.org}}
	}
	\bib{Gfan}{article}{
		author={Jensen, Anders},
		title={\texttt{\upshape gfan}: a software package for computing Gr\"obner fans and tropical varieties},
		date={2008},
		note={Version 0.3},
		eprint={\neturltilde{http://www.math.tu-berlin.de/~jensen/software/gfan/gfan.html}{http://www.math.tu-berlin.de/\~{}jensen/software/gfan/gfan.html}},	}
	\bib{Macaulay}{article}{
		author={Grayson, Dan},
		author={Stillman, Mike},
		title={\texttt{\upshape Macaulay 2}: a software system for research in algebraic geometry},
		date={2008},
		note={Version 1.1},
		eprint={\neturl{http://www.math.uiuc.edu/Macaulay2/}}
	}
	\bib{Magma}{article}{
		author={\edef\comma{,~}Computational Algebra Research Group\comma School of Mathematics and Statistics\comma University of Sydney},
		title={\texttt{\upshape MAGMA} computational algebra system},
		date={2008},
		note={Version 2.15-1},
		eprint={\neturl{http://magma.maths.usyd.edu.au/magma/}}
	}
	\bib{Polymake}{article}{
		author={Gawrilow, Ewgenij},
		author={Joswig, Michael},
		title={\texttt{\upshape polymake}: a framework for analyzing convex polytopes},
		date={2007},
		note={Version 2.3},
		eprint={\neturl{http://www.math.tu-berlin.de/polymake/}}
	}
\end{biblist}


\end{document}
